Nonlinear contractile response of actomyosin active gels to control signals

Biological systems tightly regulate their physiological state using control signals. This includes the actomyosin cytoskeleton, a contractile active gel that consumes chemical free energy to drive many examples of cellular mechanical behavior. Upstream regulatory pathways activate or inhibit actomyosin activity. However, the contractile response of the actomyosin cytoskeleton to control signals remains poorly characterized. Here we employ reconstituted actomyosin active gels and subject them to step and pulsatile activation inputs. We find evidence for a nonlinear impulse response, which we quantify via a transfer function $\delta \varepsilon / \delta g$ that relates input free-energy pulses $\delta g$ to output strain pulses $\delta \varepsilon$. We find a scaling relation $\delta \varepsilon / \delta g \sim g^{-0.3}$. The negative sign of the exponent represents a decreased effectiveness of a contracting gel in converting energy to strain. We ascribe nonlinearity in our system to a density-dependent mechanism, which contrasts strain-stiffening nonlinear responses to external stresses. Contractile response to control signals is an essential step toward understanding how information from mechanical signaling processes flow through actomyosin networks in living, and likely also synthetic, cells.

==> resources/macros.tex <==
% macros - added by James Clarke 20231018

%%%%%%%%%%%
% Needed for figures
%%%%%%%%%%%
\usepackage{epsf}

%%%%%%%%%
% Needed for lists
%%%%%%%%%
\usepackage{enumitem}

% %%%%%%%%%
% % Customize fonts
% %%%%%%%%%
% \usepackage[varg]{txfonts}
% \newcommand {\bepsilon}{\mbox{\boldmath$\epsilon$}}


%%%%%%%%%%%%%
% Define custom symbols
%%%%%%%%%%%%%
\newcommand {\ltapp}   {\stackrel {_{\normalsize<}}{_{\normalsize \sim}}}
\newcommand {\gtapp}   {\stackrel {_{\normalsize>}}{_{\normalsize \sim}}}
\newcommand {\brho}    {\mbox{\boldmath$\rho$}}
\newcommand {\bbeta}   {\mbox{\boldmath$\beta$}}
\newcommand {\btau}    {\mbox{\boldmath$\tau$}}
\newcommand {\bsigma}  {\mbox{\boldmath$\sigma$}}
\newcommand {\bft}[1]   {{\textbf #1}}
%\newcommand {\em}[1]    {{\emph{#1}}}

% DEFINE HELPFUL SYMBOL SHORTCUTS
\newcommand{\inv}{^{-1}}
\newcommand{\limit}[2]{\ensuremath{\lim_{#1}{#2}}}
\newcommand{\nlog}[1]{\ensuremath{\naturallogarithm{#1}}}
%% ARROWS
% \to already exists
\newcommand{\too}[1][]{\ensuremath{\overset{#1}{\longrightarrow}}}
\newcommand{\ot}{\ensuremath{\leftarrow}}
\newcommand{\oot}[1][]{\ensuremath{\overset{#1}{\longleftarrow}}}

\newcommand{\eq}[2]{\begin{equation}{#1}\label{#2}\end{equation}}
\newcommand{\beq}[2]{\begin{equation}{\boxed{#1}\,.}\label{#2}\end{equation}}
\newcommand{\eqs}[1]{\begin{equation*}{#1}\end{equation*}}
\newcommand{\aligneq}[2]{\begin{align}{#1}\label{#2}\end{align}}
\newcommand{\aligneqs}[1]{\begin{align*}{#1}\end{align*}}
\newcommand{\m}[1]{${#1}$}
\newcommand{\fig}[3]{
	\begin{figure}[ht]
	\centerline{\includegraphics[width={#1}\textwidth]{#2}}\label{#3}
	\end{figure}}
\newcommand{\figcap}[4]{
	\begin{figure}[ht]
	\centerline{\includegraphics[width={#1}\textwidth]{#2}}
	\caption{{#3}}\label{#4}
	\end{figure}}

% GREEK LETTERS, ETC.
\let\al\alpha
\let\be\beta
\let\gm\gamma
\let\Gm\Gamma
\let\de\delta
\let\De\Delta
\let\si\sigma
\let\Si\Sigma
\let\om\omega
\let\ka\kappa
\let\la\lambda
\let\La\Lambda
\let\ze\zeta
\let\th\theta
\let\Th\Theta
\let\vth\vartheta
\let\Om\Omega

% Set Notation Number fields
\newcommand{\R}{\ensuremath{\mathbb{R}}} %Reals
\newcommand{\C}{\ensuremath{\mathbb{C}}} %Complex
\newcommand{\Q}{\ensuremath{\mathbb{Q}}} %Rational
\newcommand{\Z}{\ensuremath{\mathbb{Z}}} %Integers
\newcommand{\N}{\ensuremath{\mathbb{N}}} %Naturals

% Parenthesis, Brackets, absolute value
\newcommand{\pa}[1]{\left(#1\right)} % encloses the argument using stretchable parentheses
\newcommand{\brac}[1]{\left[#1\right]} % encloses the argument using stretchable square brackets
%\newcommand{\brace}[1]{\left\{#1\right\}} % encloses the argument with braces
\newcommand{\vbrac}[1]{\left\langle#1\right\rangle} % encloses the argument with langle
\newcommand{\absv}[1]{\left|#1\right|} % encloses the argument using stretchable absolute value bars
\newcommand{\dabsv}[1]{\absv{\absv{#1}}}

% variations of \frac and \sfrac
\newcommand{\pfrac}[2]{\pa{\frac{#1}{#2}}} % enclosed in parentheses
\newcommand{\bfrac}[2]{\brac{\frac{#1}{#2}}} % enclosed in square brackets
\newcommand{\afrac}[2]{\absv{\frac{#1}{#2}}} % enclosed in absolute value
\newcommand{\psfrac}[2]{\pa{\sfrac{#1}{#2}}} % sfrac enclosed in parentheses
\newcommand{\bsfrac}[2]{\brac{\sfrac{#1}{#2}}} % sfrac enclosed in square brackets
\newcommand{\asfrac}[2]{\absv{\sfrac{#1}{#2}}} % sfrac enclosed in absolute value
